Selfgravitating disks in binary systems: an SPH approach -- I. Implementation of the code and reliability tests

The study of the stability of massive gaseous disks around a star in a non-isolated context is not a trivial issue and becomes a more complicated task for disks hosted by binary systems. The role of self-gravity is thought to be significant, whenever the ratio of the disk to the star mass is non-negligible. To tackle these issues we implemented, tested and applied our own Smoothed Particle Hydrodynamics (SPH) algorithm. The code (named GaSPH) passed various quality tests and shows good performances, so to be reliably applied to the study of disks around stars accounting for self-gravity. This work aims to introduce and describe the algorithm, making some performance and stability tests. It constitutes the first part of a series of studies in which self-gravitating disks in binary systems will be let evolve in larger environments such as Open Clusters.

==> comandi_personalizzati_diego.tex <==
\newcommand{\barraV}{ \ \ \ \ \ }%                  5
\newcommand{\barraX}{ \barraV \barraV}%            10
\newcommand{\barraXX}{ \barraX \barraX}%           20
\newcommand{\barraXV}{ \barraX \barraX \barraV}%   25
\newcommand{\barraXXX}{ \barraXX \barraX}%         30
\newcommand{\barraL}{ \barraXX \barraXX \barraX}%  50
\newcommand{\barraC}{ \barraL \barraL}%           100

\newcommand{\DIEtilde}{$\sim$}%
%\newcommand{\DIEtilde2}{\sim}%

\newcommand{\unmezzo}{$\frac{1}{2}$}%
\newcommand{\unterzo}{$\frac{1}{3}$}%
\newcommand{\tremezzi}{$\frac{3}{2}$}%

\newcommand{\DIEminoreuguale}{$\leq$} 
\newcommand{\DIEmaggioreuguale}{$\geq$} 
\newcommand{\DIEcirca}{$\approx$}   
\newcommand{\DIEprop}{$\propto$}  %proporzionale
\newcommand{\DIEdiv}{$\div$}  % simbolo del diviso
\newcommand{\DIEms}{$M_\odot\ $}  


\newcommand{\DIEquadrupolo}{$ \ \bar{\bar{\vec{Q}}} \ $}%
\newcommand{ \rosso}{\color{red}}
\newcommand{ \nero}{\color{black}}

\newcommand{ \rr}{\color{red}}
\newcommand{ \nn}{\color{black}}

